A Compact Delay Model for OTS Devices

This paper presents a novel compact delay model of Ovonic Threshold Switch (OTS) devices that works efficiently for circuit simulations. The internal state variable of the two terminal devices is estimated using a delay system that uses a few electrical components related to a suggested equivalent circuit of the device. Finally, we tested the proposed model against measured data from devices fabricated by Western Digital Research.

==> authors.tex <==
\section*{Authors}
\begin{wrapfigure}{l}{25mm} 
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Chawa}
\end{wrapfigure}
\par
\textbf{Mohamad Moner Al Chawa} 
%(M'2015) received the M.S. degree in 
(Member, IEEE) received the M.S. degree in advanced communication engineering from Damascus University, Damascus, Syria, in 2013, and the dual Ph.D. degree (cum laude) in electronic engineering from the Universitat de les Illes Balears (UIB), Palma, Spain, and the Universitat Politècnica de Catalunya (UPC), Barcelona, Spain, in 2018. He was a Research Assistant with the Physics Department, UIB, from 2017 to 2019. He has been a Research Associate with the Institute of Circuits and Systems, Technische Universität Dresden (TUD), since October 2019. His research interests include memristive devices and systems, nanodevice modeling, and circuit design. He was awarded an Erasmus Mundus Doctorate Grant from the Higher Education and Research Area between Europe and the Middle East ‘HERMES’ Program funded by the European Union from 2014 to 2017.
\par
\begin{wrapfigure}{l}{25mm} 
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{}
  \end{wrapfigure}\par
  \textbf{Daniel Bedau } 
  XXXXXXX XXXXXXXXX XXXX XXXXXXX XXXXXXXXXXXXXXXXXXXXXXXXX xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxx xxxxxxxxxxxx x
  \par




\begin{wrapfigure}{l}{25mm} 
\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{demir-3132278-small.png}
\end{wrapfigure}
\par
\textbf{Ahmet S. Demirkol} 
received the Ph.D. degree in electronics engineering from Istanbul Technical University, in 2014. He has been a Research Associate with the Chair of Fundamentals of Electrical Engineering, TUD, since 2019. Previously, he was the Lead Researcher in a joint project with Infineon AG at the Chair of Fundamentals of Electrical Engineering from 2015 to 2019. His current research interests cover modeling of memristors, analysis and design of memristive systems, cellular nonlinear networks, and neuromorphic circuit design, while he has a strong research experience in distortion analysis of RF switches using Volterra series, compact device modeling, analog circuit design, active network synthesis, nonlinear dynamics, and chaos.
\par
\begin{wrapfigure}{l}{25mm} 
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{}
  \end{wrapfigure}\par
  \textbf{ James W. Reiner } 
  XXXXXXX XXXXXXXXX XXXX XXXXXXX XXXXXXXXXXXXXXXXXXXXXXXXX xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxx xxxxxxxxxxxx x
  xxxxxxxx xxxxxxxxx xxxxxxxxxx xxxxxxx.
\par
%
   %%
  \begin{wrapfigure}{l}{25mm} 
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{}
  \end{wrapfigure}\par
  \textbf{ Derek A. Stewart } 
  XXXXXXX XXXXXXXXX XXXX XXXXXXX XXXXXXXXXXXXXXXXXXXXXXXXX xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxx xxxxx xxxx xxxxxxxxxxxxxxxx xxxxxxx xxxxxxxxxxxx x
\par
%%%
  \begin{wrapfigure}{l}{25mm} 
   \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{}
  \end{wrapfigure}\par
 \textbf{  Michael K. Grobis } 
  XXXXXXX XXXXXXXXX XXXX XXXXXXX XXXXXXXXXXXXXXXXXXXXXXXXX xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxxxxxxxxxxx xxxxxxx xxxxxxxxxxxx x
\par
%%%
 \begin{wrapfigure}{l}{25mm} 
    \includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{prof}
  \end{wrapfigure}\par
  \textbf{Ronald Tetzlaff }is currently a Full Professor of fundamentals of electrical engineering with TUD.
  %Technische Universität Dresden (TUD).
  His interests lie in the theory of signals and systems, system modeling and identification, Volterra systems, cellular nonlinear networks, and memristors. He is a member of the ITG, the German Society of Electrical Engineers, and the German URSI Committee. He was an Associate Editor of the IEEE Transactions on Circuits and Systems—I: Regular Papers from 1999 to 2003. He was a Distinguished Lecturer of the IEEE CAS Society from 2001 to 2002.
\par 
